Improving Blockchain Scalability with the Setchain Data-type

Blockchain technologies are facing a scalability challenge, which must be overcome to guarantee a wider adoption of the technology. This scalability issue is due to the use of consensus algorithms to guarantee the total order of the chain of blocks and of the transactions within each block. However, total order is often not fully necessary, since important advanced applications of smart-contracts do not require a total order among all operations. A much higher scalability can potentially be achieved if a more relaxed order can be exploited. In this paper, we propose a novel distributed concurrent data type, called Setchain, which improves scalability significantly. A Setchain implements a grow-only set whose elements are not ordered, unlike conventional blockchain operations. When convenient, the Setchain allows forcing a synchronization barrier that assigns permanently an epoch number to a subset of the latest elements added, agreed by consensus. Therefore, two operations in the same epoch are not ordered, while two operations in different epochs are ordered by their respective epoch number. We present different Byzantine-tolerant implementations of Setchain, prove their correctness and report on an empirical evaluation of a prototype implementation. Our results show that Setchain is orders of magnitude faster than consensus-based ledgers, since it implements grow-only sets with epoch synchronization instead of total order. Since Setchain barriers can be synchronized with the underlying blockchain, Setchain objects can be used as a sidechain to implement many decentralized solutions with much faster operations than direct implementations on top of blockchains. Finally, we also present an algorithm that encompasses in a single process the combined behavior of Byzantine servers, which simplifies correctness proofs by encoding the general attacker in a concrete implementation.

==> Incentives.tex <==
\section{Incentives}\label{sec:incentives}

We want to reward servers when they do a correct work. \capretto{and
  punish the ones that do something incorrect? }
%
So far, the only evidence of work that we have is when servers sign
the hash of epochs.  (we also discussed signing every element that is
added but it might be too expensive)
%

For each epoch that a server signed correctly (i.e., in \<theset>
\capretto{maybe we have to request it to be in epochs otherwise there is
  no incentive for servers to insert signed epochs to new epochs
  neither to return a complete a theset in a Get, so clients might
  not get the signatures? or maybe the server will return each epoch
  signed at least f+1 times os that the client can trust them?...} the
same epoch appears signed by at least f+1 servers), the server will
receive some tokens $t = (c + f(e) + g(s)) * h(s)$, where:
\begin{itemize}
   \item $c$ is a positive constant. It is used to incentive servers
     to create new epochs frequently,
   \item $e$ is the amount of ``regular'' elements that are in the
     signed epoch and $f$ is an strictly increasing function. That is,
     the more elements an epoch has the more tokens the servers get,
     so this incentives servers to do the necessary work to add new
     elements to the Setchain,
   \item $s$ is the number of servers that have inserted the epoch
     signed, $h$ is a binary function that is 0 for $s \leq f$ and 1
     for $f < s \leq n$, and $g$ is a strictly increasing
     function. Since everything is multiplied by $h(s)$ it prevents
     servers to get paid unless $f+1$ servers have also signed the
     same epoch, therefore only servers that sign correct epochs are
     rewarded.  On the other hand, the fact that $g$ is an increasing
     function creates incentives for servers to collaborate in the
     propagation of epochs signed by all other servers not only the
     first $f$ (which would create a competition between the servers
     to be in the first $f+1$ and therefore they will ignore the
     signatures from some of the other servers). Hence, when a server
     signs an epoch it not only benefits them but also all the other
     servers that have signed it.
\end{itemize}

we need to find a right balance between the functions $f$ and $g$ and
constant $c$, so that inserting elements is not too expensive for
clients while the reward for servers is big enough too keep them
participating correctly in the creation of epochs.

%
When clients insert elements they have to pay $x$ tokens for it.
%
Part of it is distributed between the servers that signed the hash of
the epoch that contains the given element and the rest is burned.
%
This prevents servers from inserting random elements as they will have
to pay more for inserting it than what they are going to receive from
the work done.
%

* Tragedy of the commons/free-rider

* Insert incorrect elements to force validation from the servers.


==> algorithms/wrapper.add.tex <==
\begin{figure}[ht]
	\begin{algorithm}[H]
    \caption{\small Wrapper for function DPO.\textbf{Add}($e$) for
algorithms~\ref{DPO-alg1},~\ref{DPO-alg-basb}, and~\ref{DPO-alg-basb3}.}
          \label{DPO-wAdd}
          \begin{algorithmic}[1]
		    \Function{WAdd}{$e$}
        \State \<call> \<DPO>.\<Add>\((e)\) in \(f+1\) different servers.
		%	\State \textbf{wait } response $ACK$ from 1 server.
			\State \<return> \<ack>
			\EndFunction
		\end{algorithmic}
	\end{algorithm}\vspace{-2em}
\end{figure}


==> algorithms/wrapper.epochinc1.tex <==
\begin{figure}[ht]
	\begin{algorithm}[H]
          \caption{\small Wrapper for function DPO.\textbf{EpochInc}$(h)$ for algorithm~\ref{DPO-alg1}.}
          \label{DPO-wEpochInc1}
          \begin{algorithmic}[1]
		    \Function{WEpochInc}{$h$}
			\State \<call> \<DPO>.\<EpochInc>\((h)\) in \(3f+1\) different servers.
		%	\State \textbf{wait } response $ACK$ from 1 server.
			\State \<return> \<call>
			\EndFunction
		\end{algorithmic}
	\end{algorithm}\vspace{-2em}
\end{figure}


==> algorithms/wrapper.epochinc23.tex <==
\begin{figure}[ht]
	\begin{algorithm}[H]
          \caption{\small Wrapper for function DPO.\textbf{EpochInc}$(h)$ in algorithms~\ref{DPO-alg-basb} and~\ref{DPO-alg-basb3}.}
          \label{DPO-wEpochInc23}
          \begin{algorithmic}[1]
		    \Function{WEpochInc}{$h$}
			\State \<call> \<DPO>.\<EpochInc>\((h)\) in \(f+1\) different servers.
		%	\State \textbf{wait } response $ACK$ from 1 server.
			\State \<return> \<ack>
			\EndFunction
		\end{algorithmic}
	\end{algorithm}\vspace{-2em}
\end{figure}


==> algorithms/wrapper.get.tex <==
\begin{figure}[ht]
  \begin{algorithm}[H]
    \caption{\small Wrapper for function DPO.\textbf{Get}().}~\label{DPO-wget}
    \begin{algorithmic}[1]
      \Function{WGet}{~}
      \State \<call> \<DPO>.\<Get>\(()\) in \(3f+1\) different servers.
        % \Comment{add identifier.}
      \State \<wait> \(2f+1\) different responses $(\THESET_i, \HISTORY_i)$ % from \(2f+1\) different servers.
      \State $stamped \leftarrow \emptyset$
      \State $h \leftarrow 0$
      \State $S \leftarrow \{ i : \text{sever } i \text{ has answered} \land K_i^{0}\}$
      \While {\(consent_{f+1}(S,\<history>,h) = E\)}~\label{DPO-bwhile}
        \State $stamped \leftarrow stamped \cup \{ \langle h, E \rangle \} $
        \State $S \leftarrow S \setminus \{ i : E \neq \<history>_i^h\}$ \Comment{remove byzantine}
        \State $h \leftarrow h+1$
        \State $S \leftarrow S \setminus \{ i : \neg K_i^{h}\}$ \Comment{remove slow server}
      \EndWhile~\label{DPO-ewhile}
      \State \(rset <- \{ e : e \text{ in at least } f+1 \text{ different sets } \THESET_i\}\)
      \State \<return> $(rset, stamped)$
      \EndFunction
		\end{algorithmic}
	\end{algorithm}\vspace{-2em}
\end{figure}

      %for algorithm 1, 2 and 3.
      % Epochs are added completely.


==> dpo-optimistic.tex <==
\section{Optimistic client for DPO}
\label{sec:wrappers-optimistic}

In Section~\ref{sec:wrappers} we described a correct client protocol
for the DPO.
%
To add an element that client must contact $f+1$ different servers to
guarantee that at least one of them will be correct, ensuring that the
element is eventually inserted in the \setchain.
%
%% Similarly, to produce an epoch change it must send requests to $f+1$
%% different servers.            
%
To know which elements have been added and which have been already
stamped in the \setchain, it must invoke $\<Get>$ in $3f+1$ different
servers, in order to receive enough responses to compute correct
$\<history>$ and $\<theset>$.

%
Here we present an alternative faster optimistic client.
%
In this approach correct servers sign cryptographically a hash of the
set of elements in an epoch, and insert it in the \setchain as an
element, see Alg.~\ref{server-sign}.
%
Observe that servers cryptographically sign each epoch and not each
element.
%
Therefore, the number of new elements added to the \setchain by the
servers is order of magnitudes smaller than the number of element in
the \setchain.
%
\input{algorithms/server-sign}
%

Alg.~\ref{optimistic} shows the optimistic client described below.
%
\input{algorithms/optimistic}
%
To insert an element $e$ in the \setchain, clients only perform
\textbf{a single} \(\<Add>(e)\) request to one server, hoping it will
be a correct server.
%
%% After waiting for some time, the client invokes an $\<EpochInc>$ in
%% \textbf{a single} server to try to get $e$ added in a new epoch, which
%% hash will be cryptographically signed and added to the \setchain by
%% the servers.
%% \marga{o asumimos que los epochInc se hacen solos cada cierto periodo?}
%
After waiting for some time, the client invokes a $\<Get>$ from
\textbf{a single} server (which again can be Byzantine) and check
whether $e$ is in some epoch whose hash appear in the \setchain signed
by (at least) $f+1$ different servers.
%
Notice that receiving a $\<history>$ in which $e$ is in an epoch is
not enough to guarantee that $e$ have been added nor stamped, because
a Byzantine server can lie in their response and since the client
receives just one response it does not have a way to tell if it is
correct or not.
%
But, since cryptographic signatures cannot be forged, and it checks
that the hash of the epoch containing $e$ was signed by at least
$f+1$, at least one correct server must have signed it, which implies
that the epoch is correct and $e$ has not been only successfully
inserted but also stamped.
% Optimistic clients can repeat the process after a timeout if the
% contacted server did not respond.

%
If we compare this client with the client presented in
\ref{sec:wrappers} we can observe that the latency between the request
to add an element and knowing it has been/will be actually added to
the \setchain is bigger in this optimistic client.
%
This is due to the fact that it needs to wait until there is enough
cryptography evidence that that things went well while the other
client by just contacting $f+1$ servers can be sure that at least one
of them is correct and therefore the element will be eventually added
to the \setchain.
%
On the other hand, this client requires only one message per $\<Add>$
and one message per $\<Get>$.
%
This reduce dramatically the number of messages sended from the client
to servers and especially between servers.
%
An $\<Add>$ request triggers a BRB.Broadcast which inside produces a
cascade of messages that is quadratic in the number of servers.
%
Hence, these two clients present a tradeoff between latency and
throughput.

